Metamorpheus: Interactive, Affective, and Creative Dream Narration Through Metaphorical Visual Storytelling

Human emotions are essentially molded by lived experiences, from which we construct personalised meaning. The engagement in such meaning-making process has been practiced as an intervention in various psychotherapies to promote wellness. Nevertheless, to support recollecting and recounting lived experiences in everyday life remains under explored in HCI. It also remains unknown how technologies such as generative AI models can facilitate the meaning making process, and ultimately support affective mindfulness. In this paper we present Metamorpheus, an affective interface that engages users in a creative visual storytelling of emotional experiences during dreams. Metamorpheus arranges the storyline based on a dream's emotional arc, and provokes self-reflection through the creation of metaphorical images and text depictions. The system provides metaphor suggestions, and generates visual metaphors and text depictions using generative AI models, while users can apply generations to recolour and re-arrange the interface to be visually affective. Our experience-centred evaluation manifests that, by interacting with Metamorpheus, users can recall their dreams in vivid detail, through which they relive and reflect upon their experiences in a meaningful way.

==> table-demographics.tex <==
\begin{table*}[!ht]
    \centering
    \begin{tabular}{ccc}
    \toprule
    \textbf{ID} & \textbf{Age} & \textbf{Gender} \\
    \midrule
    P1 &  & Male \\
    P2 &  & Female \\
    P3 & 19 & Female \\
    P4 & & Female \\
    P5 & 19 & Female \\
    P6 & & Female\\
    P7 & 20 & Female \\
    P8 & & Male 
    P9 & & Male
    P10 & & Female
    P11 & & Male
    P12 & & Male\\
    \bottomrule
    \end{tabular}
    \caption{Participant Demographics}
    \label{tab:demographics}
\end{table*}
